Automated Testing of Image Captioning Systems

Image captioning (IC) systems, which automatically generate a text description of the salient objects in an image (real or synthetic), have seen great progress over the past few years due to the development of deep neural networks. IC plays an indispensable role in human society, for example, labeling massive photos for scientific studies and assisting visually-impaired people in perceiving the world. However, even the top-notch IC systems, such as Microsoft Azure Cognitive Services and IBM Image Caption Generator, may return incorrect results, leading to the omission of important objects, deep misunderstanding, and threats to personal safety. To address this problem, we propose MetaIC, the \textit{first} metamorphic testing approach to validate IC systems. Our core idea is that the object names should exhibit directional changes after object insertion. Specifically, MetaIC (1) extracts objects from existing images to construct an object corpus; (2) inserts an object into an image via novel object resizing and location tuning algorithms; and (3) reports image pairs whose captions do not exhibit differences in an expected way. In our evaluation, we use MetaIC to test one widely-adopted image captioning API and five state-of-the-art (SOTA) image captioning models. Using 1,000 seeds, MetaIC successfully reports 16,825 erroneous issues with high precision (84.9\%-98.4\%). There are three kinds of errors: misclassification, omission, and incorrect quantity. We visualize the errors reported by MetaIC, which shows that flexible overlapping setting facilitates IC testing by increasing and diversifying the reported errors. In addition, MetaIC can be further generalized to detect label errors in the training dataset, which has successfully detected 151 incorrect labels in MS COCO Caption, a standard dataset in image captioning.

==> Data.tex <==
\section{Data Availability}\label{sec:data}

Codes for MetaIC and for re-producing all experiments results will be available at anonymous link\footnote{Hidden during review. Reviewers please refer to the supplementary materials.}. The dataset of the collected captions from six IC systems and our object source images will be available at anonymous link\footnote{Hidden during review. Reviewer please refer to the supplementary materials.}.

% Original introduction of the data availability
% All the code and dataset in {\methodname} will be open-sourced in [repository name] at http://doi.org/[doi], reference number [reference number], which can be used to reproduce our work in this paper. The code includes an object inserting method to synthesize our testing data, an implementation of {\methodname} to report the suspicious issues, and a tool to find the prospective label errors in MS COCO Caption~\cite{chen2015microsoft}. The dataset includes an image pool of 60 categories we collect from Flickr~\cite{flickr}, an object pool we extract from the collected object image pool by using Yolact++~\cite{bolya2020yolact++}, a dataset of synthesized images we produce using our object inserting technique, and the captions produced by the ICs testing on our synthesized dataset.


% Codes and datasets used in the paper have been publicly released:
% \begin{itemize}
% \item The code and data for the object inserting method will be available in [repository name] at http://doi.org/[doi], reference number [reference number], including object extraction, object resizing and object location for synthesizing the images with different overlapping ratios. We also provide our collected object images in this repository. Researchers can use this code to generate the images with different overlapping ratios as we show in this paper.

% \item The implementation of the analyzing tool of MetaIC will be available in [repository name] at http://doi.org/[doi], reference number [reference number], and we provide the captions generated by seven ICs testing on our synthesized dataset in this repository. Researchers can use the analyzing tool to report the suspicious issues.

% \item The tool we use to find GT labels will be available in [repository name] at http://doi.org/[doi], reference number [reference number], researchers can use this tool to find suspicious label errors in MS COCO Caption.

% \end{itemize}

% We will provide the object inserting code, including object extraction, object resizing and object location for synthesizing the images with different overlapping ratios. We will provide the captions experiments and our analyzing code to report the suspicious issues, along with the captions of the two APIs and five models, which we use in our experiments. We will provide the list of label errors in MS COCO Caption and our tool to find that erroneous labels.

==> Discussion.tex <==
\bx {\section{Discussion}\label{sec:discuss} }

\subsection{Hyper-parameter Setting}

{\methodname} has two groups of hyper-parameters: object resizing parameters and overlapping ratio interval parameters. We tune the value of these parameters on a subset of the validation dataset of COCO Caption and it leads to high precision when we use the test dataset as seeds in {\methodname}.

\subsubsection{Object resizing parameters} 
The inserted object cannot be too large or too small because we need to make it a salient object while not affecting the saliency of the original objects. 
We considered two situations (<40\% v.s. >=40\%) because we found that if the largest original object occupies a large area, the inserted object should not be too large; otherwise, it is difficult to control the overlapping ratios between it and the original objects, which incurs much more iterations in the object insertion algorithm. Based on grid search, we found 40\% provided the best result in terms of the naturalness of the synthesized images. We also use grid search to tune as $\alpha$ and $\beta$ on the same set of images.

\subsubsection{Overlapping ratio interval parameters} 
We intend to generate images with different overlapping ratios because in practice the objects could overlap with each other. Thus, we set $ratio_{max}=0.45$ and $n=4$ to generate different overlapping ratio intervals.
% In practice, developers can pick different overlapping ratios according to their needs. For example, if developers intend to have intervals [0], (0, 0.10], and (0.10, 0.20], which means that the overlapping ratios of the synthesized images will fall into these three intervals, they can set $ratio_{max}=0.20$ and $n=3$.

\subsection{Naturalness of Synthetic Image}

Some synthesized images are different from the images in the training set. However, the synthesized images are useful and the incorrect captions of these images are issues/errors because of the following reasons. 
First, generalization ability is important for AI models. For example, if there is an image “a bird flying in the sky” and an image “a monkey on the tree” in the training set, it is reasonable to expect the model to learn the correct caption for an image “a monkey flying in the sky”. 
Second, it is also reasonable to expect AI software to be robust against unexpected inputs. There was a severe car accident due to lack of robustness~\cite{accident_white_car}.
Third, the ability of captioning synthesized images is also important. Nowadays, in addition to real images (camera images), there are a lot of synthesized images (e.g., images in the comics and images edited by software like Photoshop) in our lives. Thus, similar to camera images, we also need to use IC software to understand/summarize synthesized images. 


\subsection{Recall Rate}
Compared to precision, recall rate is not important in our experiment. This is because that it is difficult to find all the bugs of the AI models. Therefore, we only compute the recall rate for Attention~\cite{xu_show_2015}, where {\methodname} achieve a high recall rate of 99.3\% over all the overlapping ratios.
% \begin{itemize}
%     \item 
% \end{itemize}
% Therefore, we only compute the recall rate for Attention~\cite{xu_show_2015}

==> ISSTA2022_IC (2)/Conclusion.tex <==
\section{Conclusion}\label{sec:con}

In this paper, we propose the first black-box testing approach, {\methodname}, for validating image captioning systems. The distinct benefits of {\methodname} are its simplicity and generality, and thus wide applicability. {\methodname} can effectively disclose many captioning errors. In our experiments, {\methodname} successfully reports 16,825 erroneous issues in six IC systems with high precision (84.9\%-98.4\%) revealing 17,380 captioning errors. In addition to the main focus of this paper (\textit{i.e.}, testing), to further understand the reported errors, we visualize the attention of objects in CNN-RNN-Based ICs and the predictions of Faster R-CNN used in VLP ICs, which explores the major root causes behind. We also show that {\methodname} can be adapted to find errors in the standard dataset of image captioning, indicating its potential in further enhancing the reliability of IC systems. For future work, we plan to extend {\methodname} by considering other kinds of caption constituents (\textit{e.g.}, verbs). We will also explore automated error detection for standard datasets, which we regard as an important future direction.
% We will continue to advance the module of {\methodname}, e.g. constructing word dict which maps the synonyms to our object classes to eliminate some of {\methodname}'s false postive issues et al. 
% Meanwhile, we intend to adapt {\methodname} to detect more label errors in different multimodal datasets to help developing high-quality data for researching multimodal tasks.

==> ISSTA2022_IC (2)/Data.tex <==
\section{Data Availability}\label{sec:data}

Codes for MetaIC and for re-producing all experiments results will be available at anonymous link\footnote{Hidden during review. Reviewers please refer to the supplementary materials.}. The dataset of the collected captions from six IC systems and our object source images will be available at anonymous link\footnote{Hidden during review. Reviewer please refer to the supplementary materials.}.

% Original introduction of the data availability
% All the code and dataset in {\methodname} will be open-sourced in [repository name] at http://doi.org/[doi], reference number [reference number], which can be used to reproduce our work in this paper. The code includes an object inserting method to synthesize our testing data, an implementation of {\methodname} to report the suspicious issues, and a tool to find the prospective label errors in MS COCO Caption~\cite{chen2015microsoft}. The dataset includes an image pool of 60 categories we collect from Flickr~\cite{flickr}, an object pool we extract from the collected object image pool by using Yolact++~\cite{bolya2020yolact++}, a dataset of synthesized images we produce using our object inserting technique, and the captions produced by the ICs testing on our synthesized dataset.


% Codes and datasets used in the paper have been publicly released:
% \begin{itemize}
% \item The code and data for the object inserting method will be available in [repository name] at http://doi.org/[doi], reference number [reference number], including object extraction, object resizing and object location for synthesizing the images with different overlapping ratios. We also provide our collected object images in this repository. Researchers can use this code to generate the images with different overlapping ratios as we show in this paper.

% \item The implementation of the analyzing tool of MetaIC will be available in [repository name] at http://doi.org/[doi], reference number [reference number], and we provide the captions generated by seven ICs testing on our synthesized dataset in this repository. Researchers can use the analyzing tool to report the suspicious issues.

% \item The tool we use to find GT labels will be available in [repository name] at http://doi.org/[doi], reference number [reference number], researchers can use this tool to find suspicious label errors in MS COCO Caption.

% \end{itemize}

% We will provide the object inserting code, including object extraction, object resizing and object location for synthesizing the images with different overlapping ratios. We will provide the captions experiments and our analyzing code to report the suspicious issues, along with the captions of the two APIs and five models, which we use in our experiments. We will provide the list of label errors in MS COCO Caption and our tool to find that erroneous labels.

==> ISSTA2022_IC (2)/Discussion.tex <==
\bx {\section{Discussion}\label{sec:discuss} }

\subsection{Hyper-parameter Setting}

{\methodname} has two groups of hyper-parameters: object resizing parameters and overlapping ratio interval parameters. We tune the value of these parameters on a subset of the validation dataset of COCO Caption and it leads to high precision when we use the test dataset as seeds in {\methodname}.

\subsubsection{Object resizing parameters} 
The inserted object cannot be too large or too small because we need to make it a salient object while not affecting the saliency of the original objects. 
We considered two situations (<40\% v.s. >=40\%) because we found that if the largest original object occupies a large area, the inserted object should not be too large; otherwise, it is difficult to control the overlapping ratios between it and the original objects, which incurs much more iterations in the object insertion algorithm. Based on grid search, we found 40\% provided the best result in terms of the naturalness of the synthesized images. We also use grid search to tune as $\alpha$ and $\beta$ on the same set of images.

\subsubsection{Overlapping ratio interval parameters} 
We intend to generate images with different overlapping ratios because in practice the objects could overlap with each other. Thus, we set $ratio_{max}=0.45$ and $n=4$ to generate different overlapping ratio intervals.
% In practice, developers can pick different overlapping ratios according to their needs. For example, if developers intend to have intervals [0], (0, 0.10], and (0.10, 0.20], which means that the overlapping ratios of the synthesized images will fall into these three intervals, they can set $ratio_{max}=0.20$ and $n=3$.

\subsection{Naturalness of Synthetic Image}

Some synthesized images are different from the images in the training set. However, the synthesized images are useful and the incorrect captions of these images are issues/errors because of the following reasons. 
First, generalization ability is important for AI models. For example, if there is an image “a bird flying in the sky” and an image “a monkey on the tree” in the training set, it is reasonable to expect the model to learn the correct caption for an image “a monkey flying in the sky”. 
Second, it is also reasonable to expect AI software to be robust against unexpected inputs. There was a severe car accident due to lack of robustness~\cite{accident_white_car}.
Third, the ability of captioning synthesized images is also important. Nowadays, in addition to real images (camera images), there are a lot of synthesized images (e.g., images in the comics and images edited by software like Photoshop) in our lives. Thus, similar to camera images, we also need to use IC software to understand/summarize synthesized images. 


\subsection{Recall Rate}
Compared to precision, recall rate is not important in our experiment. This is because that it is difficult to find all the bugs of the AI models. Therefore, we only compute the recall rate for Attention~\cite{xu_show_2015}, where {\methodname} achieve a high recall rate of 99.3\% over all the overlapping ratios.
% \begin{itemize}
%     \item 
% \end{itemize}
% Therefore, we only compute the recall rate for Attention~\cite{xu_show_2015}

==> ISSTA2022_IC (2)/Experiment.tex <==
\section{Evaluation}\label{sec:exper}

\subsection{Experimental Setup and Dataset}

\begin{table*}[ht]
		\centering
		\caption{Precision (true positives/suspicious issues) of Deeptest~\cite{tian_deeptest_2018} and {\methodname} on one paid API and five models.}
% 		\includegraphics[width=0.88\linewidth]{Figs/final_precision_table.pdf}
		\includegraphics[width=0.95\linewidth]{Figs/deeptest_metaic.pdf}
		\label{fig:table_precision}
\end{table*}

\subsubsection{Experimental environments}
 All experiments are run on a Linux workstation with an 8 core AMD Ryzen 5800X 4.8GHz Processor, 64GB DDR4 2666MHz Memory, and GeForce RTX 3090 GPU. The Linux workstation is running 64-bit Ubuntu 20.04.2 LTS with Linux Kernel 5.11.0. For POS tagging, we use the XPOS implemented in Stanza,\footnote{https://stanfordnlp.github.io/stanza/} an NLP Package powered by Stanford NLP Group.

\subsubsection{Dataset}
To show that {\methodname} can work effectively on different image sources, we collect object source images from Flickr~\cite{flickr} and background images from MS COCO Caption~\cite{chen2015microsoft}, a standard dataset in image captioning field. For MS COCO Caption Dataset, we focus on the images whose class names are single words (60 out of 80) because the POS tagging technique can only assign POS to single words. 
It only requires decent engineering effort to generalize {\methodname} to class names containing multiple words. All the code and datasets in this paper will be open-source.
% , we argue that using a subset of the complete COCO dataset can successfully report tens of thousands of erroneous issues.

\subsection{Precision}
{\methodname} automatically reports suspicious issues, where each issue contains a pair of images and their captions $(I(b), I(i'))$. 
Therefore, the effectiveness lies in how precise the reported issues are. In this section, we try to answer the following question: how many of the reported issues contain real captioning errors. We test one well-known IC API: Microsoft Azure API, and five IC models: Attention~\cite{xu_show_2015}, $Oscar_B$, $Oscar_L$~\cite{li_oscar_2020}, $VinVL_B$, $VinVL_L$~\cite{zhang_vinvl_2021}. In this experiment, we set $ratio_{max}=45\%$ and $n=4$ to balance the diversity of the test cases (in terms of the overlapping ratio) and the test case quality. We believe this parameter setting can be used in other datasets in general because the MS COCO Caption contains diverse images (different sizes and salient objects). 
We use {\methodname} to randomly generate 1,000 background-object pairs from MS COCO Caption and our object corpus, and construct 1,000 synthesized images for every overlapping ratio interval.
After synthesizing the images, we obtain 4,000 image pairs $(b, i')$. We collect 4,000 caption pairs $(I(b), I(i'))$ from each of the IC systems under test. Based on these caption pairs, {\methodname} returns a list of suspicious issues. 

We are the first to test IC systems so there are no available baselines. Intuitively, the metamorphic testing techniques for simpler tasks that also take images as input could be adapted to testing IC systems. Thus, we adopt Deeptest~\cite{tian_deeptest_2018}, a metamorphic testing technique for image classifier in our precision experiment. Specifically, we use four image transformations in Deeptest (blur, brightness, contrast, shear) and check whether the image pair share the same caption. We use the same background images as the experiment setting of {\methodname} to synthesize 4,000 image pairs $(b, i')$, and collect 4,000 caption pairs $(I(b), I(i'))$ from the IC systems.

To verify the results, two authors manually inspect all the suspicious issues separately following the instructions on data labeling in MS COCO paper~\cite{chen2015microsoft}, including "Describe all the important parts of the scene", "Do not describe things that might have happened
in the future or past", \textit{etc.} During this manual analysis, all disagreements were discussed until a consensus was reached. The results of this phase have a Cohen's kappa of 0.822, showing a substantial-level of agreement~\cite{mchugh2012interrater}.

%and collectively decide whether an issue contains captioning error(s) or not. 

\subsubsection{Evaluation Metric}
If the caption pair $p=(I(b), I(i'))$ is reported as suspicious issue, and $I(b)$ or/and $I(i')$ contains captioning error(s), then we set $error(p)$ to be true, otherwise we set $error(p)$ to be false. Given a list of suspicious issues, the precision is calculated by:
\begin{equation}
    Precision = \frac{\sum_{p\in P}{error(p)}}{|P|},
\end{equation}
where $P$ are the suspicious issues reported by {\methodname} and $|P|$ is the number of the suspicious issues.

% We test the effect of perturbation by increasing the intersection region of inserted objects and the largest object in the background image
% \begin{table}[ht!]
% \centering
% \begin{tabular}{||c c c c c||} 
%  \hline
%  IC Method & $ratio_0$ & $ratio_1$ & $ratio_2$ & $ratio_3$ \\ [0.5ex] 
%  \hline
%  \hline
%  Neural-Talk-2 & 0.986 & 0.986 & 0.988 &0.988 \\ 
%  Show-Attend-Tell & 0.983 & 0.975 & 0.986 &0.977 \\
%  $Oscar_B$ & 0.903 & 0.913 & 0.908 & 0.923 \\
%  $Oscar_L$ & 0.921 & 0.924 & 0.916 & 0.905 \\
%  $VinVL_B$ & 0.854 & 0.846 & 0.872 & 0.868 \\
%  $VinVL_L$ & 0.859 & 0.860 & 0.851 & 0.854 \\ 
%  Microsoft Azure API & 0.966 & 0.962 & 0.971 & 0.971 \\[1ex] 
%  \hline
% \end{tabular}

% \caption{Precision of {\methodname} tested on several ICs\pj{add a top row named ratio, then replace the current "ratio0" row with the ratio values: 0.45, 0.3, ..}}
% \label{table:1}
% \end{table}

% \begin{figure*}[ht]
% 		\centering
% 		\includegraphics[width=1.0\linewidth]{Figs/final_precision_table.pdf}
% 		\caption{Precision of {\methodname} tested on several ICs}
% 		\label{fig:table_precision}
% \end{figure*}

\subsubsection{Results}
The results are presented in Table~\ref{fig:table_precision}, the precision of {\methodname} and Deeptest~\cite{tian_deeptest_2018} on one API and five models. 
The precision of {\methodname} ranges from 84.9\% to 98.4\%, while Deeptest's precision ranges from 12.9\% to 41.2\%. 
Specifically, {\methodname} achieves a precision of (96.1\%-97.4\%) on Microsoft Azure API, and a precision of (84.9\%-98.4\%) on the five IC models.
The results demonstrate that {\methodname} is much more precise in testing IC systems than existing metamorphic testing techniques for systems that also take images as input.
In addition, {\methodname} reports much more erroneous issues. Specifically, {\methodname} reports 535 to 948 erroneous issues, while Deeptest reports 36 to 245.
{\methodname} successfully report 16,825 erroneous issues, which contains a total number of 17,380 captioning errors.
Specifically, out of the 16,825 erroneous issues reported, 120 issues are reported because of captioning errors in the original images.
Note that the comparison between {\methodname} and Deeptest is not apple-to-apple as Deeptest was originally designed for testing image classifiers.
We regards Deeptest as a baseline here for the completeness of discussion.
The images synthesized by {\methodname} are diverse.
From the table, we can observe that {\methodname} consistently achieves high precision under different overlapping ratios, showing the effectiveness of our object resizing and location tuning algorithms. 
For example, when we use {\methodname} to test the Microsoft Azure API~\cite{miocrosoft_azure_api}, the precision values for $\{ratio_0, ratio_1, ratio_2, ratio_3\}$ are $\{96.6\%, 96.1\%, 96.5\%, 97.4\%\}$, respectively. 
% The high precision for various overlapping ratios shows that {\methodname} consistently performs well in all the experimental settings, further demonstrating the wide-applicability of {\methodname}.
% The variance of precision may be due to the variance of the vulnerability of these ICs. Some ICs are more vulnerable, thus the caption pair produced by these ICs may be undermined more easily. 
% However, {\methodname} still achieves 84.6\% on the SOTA IC $VinVL_L$.

\subsubsection{False positives}
To further understand the results, we categorize the false positives of {\methodname} and discuss the prospective solutions for them.
Although {\methodname} achieves very high precision in our evaluation, we still encounter some false positives. We manually inspect the false positives and present three typical examples in Fig.~\ref{fig:false_positive}. 
First, after inserting a bird into the background image, the caption describes the "bird" as "parrot", which is correct because parrots are subspecies of birds. 
However, our class set does not contain "parrot", leading to a false positive. Second, after inserting a cow into the background image, the depiction of the person changes from "person" to "woman". A dictionary containing more object types can effectively reduce these two kinds of false positives.
Third, "a pair of scissors" is regarded as an incorrect singular-plural form of "scissors" by our method, while in modern English, the word "scissors" has no singular form, leading to the false positive. In the future, adopting a more advanced POS tagging tool or maintaining a dictionary of words of special singular-plural form can help.


\begin{figure}[ht]
		\centering
		\includegraphics[width=1.0\linewidth]{Figs/False_Positive.pdf}
		\caption{False positives reported by {\methodname}.}
		\label{fig:false_positive}
\end{figure}

\begin{figure*}[ht]
		\centering
% 	\includegraphics[width=0.9\linewidth]{Figs/IC_errors.pdf}
	\includegraphics[width=0.94\linewidth]{Figs/xieti_IC_errors.pdf}
	\caption{Examples of captioning errors reported by {\methodname}.}
		\label{fig:error_cases}
	\vspace{4ex}
\end{figure*}

\begin{table*}[ht]
		\centering
		\caption{Ablation study of the metamorphic relations.}
% 		\includegraphics[width=0.88\linewidth]{Figs/mr_ablation.pdf}
		\includegraphics[width=0.99\linewidth]{Figs/mr_ablation.pdf}
		\label{fig:table_ablation}
\end{table*}

\subsection{Erroneous Captions}
{\methodname} is capable of finding three kinds of captioning errors: 
\begin{itemize}
  \item \textbf{Classification error} is an error that IC systems provide an incorrect class name for an object, for instance, an erroneous caption depicts an airplane as a skateboard.
  \item \textbf{Recognition error} is an error that IC systems omit the description of a salient object in the image.
  \item \textbf{Single-plural error} is an error that IC systems return the incorrect singular-plural form of an noun in the caption. For example, an erroneous caption gives a depiction "bananas" when there is only one banana in the image.
\end{itemize}

To provide a glimpse of the diversity of the uncovered errors, this section highlights examples for all the three kinds of errors in Fig.~\ref{fig:error_cases}.
% We have shown several erroneous caption cases in Fig.~\ref{fig:error_cases}, involving the aforementioned three cases, and use three cases for each category of errors. 
The first column corresponds to the classification errors, \textit{e.g.}, the caption in the first row uses "a couple of zebra" to describe the image including a sheep and a zebra, and the caption of the second row incorrectly describes the bird as a person in a garment. The second column corresponds to the recognition errors, where the caption of the first row misses the depiction of a dog near two horses, and the caption of the second row omits the sheep in a group of zebras. The third column shows the errors of singular-plural form, where the caption of the first row describes a single banana as bananas, and the caption of the second row depicts a single elephant as two elephants.
% We have shown several erroneous caption cases in Fig.~\ref{fig:error_cases}, involving the aforementioned three cases, and use three cases for each category of errors. The first column corresponds to the classification errors, e.g., the caption in the first row uses "a couple of zebra" to describe the image including a sheep and a zebra, the caption of the second row ridiculously describes the bird as a person in a garment, and the caption in the third row describes the elephant as the bird. The second column corresponds to the recognition errors, where the caption of the first row misses the depiction of a dog near two horses, the caption of the second row omits the sheep in a group of zebras, and the caption of the third row misses the cake near the person. The third column shows the errors of singular-plural form, where the caption of the first row describes a single banana as bananas, the caption of the second row depicts a single elephant as two elephants, and the caption of the third row depicts two dogs as a dog.
% E.g., for the first image in the third row, the caption "a couple of people riding a wave on a surfboard" misclassifies the pizza as a person, thus it encounters classification error. For the first image of the first row, the caption "a black and white cat sitting on a bed in a window" only depicts one cat while omitting another cat besides it, indicating the caption encounters recognition error. For the second image in the first row, the caption "a group of elephants and two bears" depicts that there is a group of elephants, while there is only one elephant in this image, thus this caption encounters singular-plural form error.

\subsection{Ablation Study}
We conduct the ablation study to evaluate the effectiveness of the two metamorphic relations we propose.
From Table~\ref{fig:table_ablation} we can see that the precision of $MR_1$ and $MR_1+MR_2$ is very close to each other in most cases.
Sometimes, the precision will be slightly decreased when we use $MR_1+MR_2$, while we will report more erroneous issues.
For example, for the $Oscar_B$ model with 45\% overlapping ratio, precision is decreased from 93.5\% to 92.2\%.
However, with $MR_1+MR_2$, we can find 35 more erroneous issues than only using $MR_1$, which shows that $MR_2$ is useful and necessary.

\subsection{Case Study on IC Errors via Visualization}
To better understand the reported captioning errors and explore the potential root causes, in this section, we conduct visualization experiments. Specifically, we try to answer the question: "why the IC systems return incorrect captions given the synthesized images?" We visualize the errors in both CNN-RNN-Based IC systems (via attention of the generated object words) and VLP IC systems (via the prediction of faster R-CNN). 

\subsubsection{CNN-RNN-Based IC}
For CNN-RNN-Based IC, we explore errors in Attention~\cite{xu_show_2015} because it achieves high accuracy among all the CNN-RNN-Based ICs. We visualize the attention mechanism as it is the most important component of the model. 
Specifically, we intend to show how different overlapping ratios would affect the attention mechanism and the caption.

In Fig.~\ref{fig:show_bear_horse}, we present the attention mask changes after inserting an object to the original background image. 
We could observe that, at the beginning, the black bear is correctly captioned in the background image. However, when we insert the horse into the background image with different overlapping ratios ($n=4$, $ratio_{max}=45\%$), we find that the captions become incorrect. For $ratio_0$ and $ratio_1$, the black horse is misclassified as a black bear. For $ratio_2$, the black horse and black bear have been both recognized as black sheep. For $ratio_3$, the black bear is misclassified as black horse. The second row of Fig.~\ref{fig:show_bear_horse} shows the attention masks generated by the model, which serves as an important component in its captioning process. By observing the attention masks of $ratio_0$ and $ratio_1$, we can see that the attention masks for the two words of "bear" in the caption mistakenly highlight the regions of both the horse and the bear. This indicates that the captioning error is likely to be caused by model's attending to incorrect region. Thus, research on improving the attention mechanism in demand.
% There are some other failure cases of Show, Attend and Tell shown Fig.~\ref{fig:show_other_two}, from which we could see that different overlapping ratios cause the IC to encounter different errors, thus proving that our object inserting method provides more comprehensive testing data for IC task.


\begin{figure*}[ht]
		\centering		\includegraphics[width=0.95\linewidth]{Figs/bear_horse_mask.pdf}
		\caption{Attention mechanism fails to depict the images.}
		\label{fig:show_bear_horse}
\end{figure*}

% \begin{figure*}[ht]
% 		\centering
% 		\includegraphics[width=1.0\linewidth]{Figs/showattend_another_couple_error.pdf}
% 		\caption{Other failure cases and their attention masks}
% 		\label{fig:show_other_two}
% \end{figure*}

\begin{figure*}[ht]
		\centering
		\includegraphics[width=1.0\linewidth]{Figs/newtwo_vlp_purturbation.pdf}
% 		\includegraphics[width=1.0\linewidth]{Figs/twoimage_vlp_perturbation.pdf}
		\caption{Errors caused by the first component (a)(b) and the second component (c) in VLP IC.}
		\label{fig:vlp_fe_errors}
\end{figure*}

\subsubsection{Perturbation to VLP IC}
% If we only consider the situation that the objects don't overlap with each other, we couldn't get to know that IC may break down under the circumstance of $ratio_3$ shown in Fig.~\ref{fig:vlp_fe_errors}. 
{\methodname} also reports many erroneous captions produced by VLP ICs. Specifically, we choose a typical VLP IC model $Oscar_B$ and conduct visualization experiment to show the vulnerabilities of the two components of VLP ICs, including Faster R-CNN in the first stage and BERT in the second stage. 
By comparing Fig.~\ref{fig:vlp_fe_errors} (a) with Fig.~\ref{fig:vlp_fe_errors} (b), we show an example where its erroneous caption is caused by Faster R-CNN (the first component). 
We draw the bounding boxes produced by the Faster R-CNN of $Oscar_B$ for the background and the synthesized image. 
For clarity, we only draw the bounding boxes for the object in the image. 
The caption produced by $Oscar_B$ is correct for the background image.
However, for the synthesized image, the caption describes a single giraffe as "a couple of giraffes", resulting in an error of singular-plural form. 
We could observe that the bounding boxes for background image are of high accuracy. 
However, the bounding box of the giraffe in the synthesized image and that of the horses have a big overlap. 
The part of the image framed by the bounding box will be encoded into region-feature, which acts as the major input to the second component of $Oscar_B$.
The second component uses region features and the corresponding tags (\textit{e.g.}, "giraffe") to generate the caption.
Specifically, $Oscar_B$ concatenates the tag "giraffe" with the region-feature for cross-modal representation learning.
We think the erroneous depiction of "a couple of giraffes" could be caused by the low-quality region-feature of "giraffe" (\textit{i.e.}, the sub-optimal bounding box). 
It overlaps a lot with the horses, and thus $Oscar_B$ captions one of the horses as a giraffe. 

% \begin{figure*}[ht]
% 		\centering
% 		\includegraphics[width=1.0\linewidth]{Figs/newtwo_vlp_purturbation.pdf}
% % 		\includegraphics[width=1.0\linewidth]{Figs/twoimage_vlp_perturbation.pdf}
% 		\caption{Errors caused by the first component (a)(b) and the second component (c) in VLP IC.}
% 		\label{fig:vlp_fe_errors}
% \end{figure*}

The visualization experiment also shows that the erroneous captions may be caused by the glitches in the BERT module the second component of VLP ICs. 
As shown in Fig.~\ref{fig:vlp_fe_errors} (c), the bounding boxes of the objects in the image are of high accuracy, while the generated sentence omits the description of the bowl on the frisbee. 
The visualization case study indicates that {\methodname} can report captioning errors cause by both the first component (image) and the second component (text).


\subsection{Finding Labeling Errors in the Training Corpus}

Labeling errors in the training corpus has been a prevalent and severe problem in machine learning and deep learning. Even the most famous Datasets have errors in their labels, such as ImageNet~\cite{krizhevsky2012imagenet}, CIFAR~\cite{krizhevsky2009learning}, and MNIST~\cite{deng2012mnist}. Several methods~\cite{sambasivan2021everyone,zhang2017improving} have been proposed to tackle this problem, mainly focusing on noises in the data. 
Recently, AI software applications are approaching human-level performance.
% , such as the classification model~\cite{he2015delving} that surpasses human on ImageNet
For IC task, Hu \textit{et al.}~\cite{hu_vivo_2020} claims that their model has achieved a better result than human in terms of CIDEr~\cite{vedantam2015cider} score in Nocaps~\cite{agrawal2019nocaps} task. 
Given that these models have been well trained on the existing corpora, fixing labeling errors in these corpora is a reasonable way to further improve their performance. 
In this section, we explore whether it is possible to adapt the high-level idea of {\methodname} detecting labelling errors in a standard dataset MS COCO Caption~\cite{chen2015microsoft}.

Specifically, denote $GT(b)$ as the label caption of image $b$ in MS COCO Caption, we have a tuple $(I(b), I(i'), GT(b))$.
Denote the common object class set between $I(b)$ and $I(i')$ as $Set_{invar}$:
\begin{equation}
    Set_{invar} = Set(I(b)) \cap Set(I(i')),
\end{equation}
Intuitively, objects classes in both $(I(b)$ and $I(i')$ imply the important objects in the image. We denote the object class set of $GT(b)$ as $Set(GT(b))$, it should satisfy the relation that:
\begin{equation}
    Set_{invar} \subset Set(GT(b)).
\end{equation}
Otherwise, $GT(b)$ may depict image $b$ improperly since it is likely to miss important objects in its caption. 
We map the object class to their super-category defined in MS COCO Caption and use the super-category in the aforementioned method.

We choose ten object classes $\{dog, cat, sheep, truck, cow, zebra,\\ elephant, horse, frisbee, bird\}$, construct 6,662 tuples of $(I(b), I(i'), \\GT(b))$, and try to find erroneous labels of these classes in MS COCO Caption. 
By using this technique adapted from {\methodname}, we have found 151 caption errors, using only a small portion of the data in MS COCO Caption.
% within just a small part of MS COCO Caption. 
We present examples of incorrect label errors in Fig.~\ref{fig:gt_error_cases}, including typos, misclassification error, "no-image" error, \textit{etc.} 
For example, caption (a) in the first row mistakenly writes "at" rather than "cat"; caption (c) mistakenly describe a "frisbee" as a "pizza"; caption (e) is a complain message rather than a caption; and caption (d) incorrectly depicts a "dog" as a "man". 

Given that the performance of deep learning models mainly depends on the model structure and the parameters learned from the training dataset, we believe the labeling errors we find with {\methodname} indicate the usefulness and wide applicability in enhancing the robustness of IC software.
Thus, it reflects the practical relevance of {\methodname}. The 151 labeling errors are found from 6,662 captioned images in the training data.
We believe our approach can detect more errors on a larger input set. 
Although finding labeling errors is not the main focus of this paper, we think the experiment demonstrates the wide-applicability of {\methodname}.
% These may be disastrous results if the AI models are trained on the dataset with these erroneous labels, especially for some security-sensitive areas.

\begin{figure}[ht]
		\centering
		\includegraphics[width=1\linewidth]{Figs/gt_label_errors.pdf}
		\caption{Labeling errors in MS COCO Caption~\cite{chen2015microsoft} reported by {\methodname}.}
		\label{fig:gt_error_cases}
\end{figure}

% \subsection{Failure Cases and Discussion}

\subsection{Retraining with Erroneous Issues}
To explore whether the erroneous issues reported by {\methodname} can be utilized to improve IC systems, we re-label the erroneous issues following the labeling standard of MS COCO Caption~\cite{chen2015microsoft}, and fine-tune the $Oscar_B$ model. 
Specifically, we add the re-labeled synthesized images to MS COCO Caption and perform fine-tuning for 40K steps. 
We follow the publicly available splits\footnote{https://cs.stanford.edu/people/karpathy/deepimagesent/} as in the original Oscar paper~\cite{li_oscar_2020} and use our synthesized images as the augmented data in the training set.

Table~\ref{fig:table_finetune} presents the results. 
We can observe that BLEU-4 increases by 1.2\%, METEOR increases by 3.7\%, CIDEr increases by 2.5\%, and SPICE increases by 8.8\%. Specifically, the SPICE~\cite{anderson2016spice} has a system-level correlation of 0.88 with human judgements on MS COCO~\cite{lin2014microsoft}. 
% According to a survey of IC systems (Table 2 in \cite{stefanini2021show}), our improvement of the four score are significant, including BLEU-4 increasing by 1.2\%, METEOR increasing by 3.7\%, CIDEr increasing by 2.5\%, and SPICE increasing by 8.8\%.
% Specifically, the SPICE~\cite{anderson2016spice} has a system-level correlation of 0.88 with human judgements on MS COCO~\cite{lin2014microsoft}. 
According to a survey of IC systems (Table 2 in \cite{stefanini2021show}), our improvement of the four score are significant.
In addition, we can see that except for BLEU-4, the other scores of $Oscar_{B-Fintune}$ are higher than $Oscar_L$.
The fine-tuned model achieves competitive performance with much fewer parameters and less training time.
The results indicate that the captioning errors in the synthetic images can be utilized to further improve the performance of IC systems, both in efficiency and accuracy, demonstrating its practical relevance.
% Thus, the erroneous issues reported by {\methodname} can be used to improve IC systems.
Note that although improving IC system using test cases is an interesting and important topic, it is not the focus of this paper. Thus, we regard it as a promising future direction.
% The improvement of the fine-tuned model compared with the original Oscar base model has shown the value of the erroneous issues reported by {\methodname}. 
% The retraining experiment also shows that our synthesized images serve as a good data augment method to enhance the ability of IC models. 

\begin{table}[ht]
		\centering
		\caption{Performance of fine-tuned model.}
		\includegraphics[width=1\linewidth]{Figs/finetune.pdf}
		\label{fig:table_finetune}
\end{table}


% \subsection{Limitations and Threats to validity}
% \bx{MetaIC has some limitations. First, although we have designed algorithms to resize and locate the inserted objects, it is still possible that the inserted object will not be salient or it impairs the saliency of the original objects, making the synthesized image difficult for human to recognize. Second, even though the NLP technique XPOS we adopt in MetaIC has high accuracy, it may generate wrong assignment of word forms, which makes MetaIC less precise. Third, we currently focus on reporting the captioning errors about the nouns, so that MetaIC cannot report the errors about the erroneous relationship between the objects, which we regard as important future work. }

==> ISSTA2022_IC (2)/Introduction.tex <==

\section{Introduction}\label{sec:intro}

% \ph{a paragraph about how important image captioning is and how popular it is.}

\begin{figure*}[ht]
		\centering
		\includegraphics[width=1.0\linewidth]{Figs/MRs_Show.pdf}
		\caption{ Examples of background images, generated images, and the corresponding captions. Words of salient objects are marked in blue. Words indicating the violation of {\methodname}'s MRs are marked in red.}
		\label{fig:how_MRs_work}
\end{figure*}



Image captioning (IC) systems aim to automatically generate a brief depiction of the salient objects in an image (real or synthetic). 
In recent years, the performance of IC systems~\cite{karpathy2015deep, vinyals_show_2015, xu_show_2015, li_oscar_2020, hu_vivo_2020, zhang_vinvl_2021} have improved significantly due to the rapid development of the underlying deep neural networks, such as convolutional neural networks (CNN)~\cite{ren2015faster, he2016deep} for image feature extraction and language models~\cite{hochreiter1997long,devlin2018bert} for caption generation based on these features.
The SOTA IC models have reached or even surpassed human-level performance (\textit{e.g.}, VIVO~\cite{hu_vivo_2020}) in terms of CIDEr score~\cite{vedantam2015cider}.
Thus, IC systems have been increasingly integrated into our daily lives.
Typical examples include generating captions for massive social media photos~\cite{ic2socialnetwork}, visually-impaired people's artificial intelligence (AI) assistants~\cite{ic2impariment, ic2impariment_2}, and the acceleration of various manual image labeling tasks~\cite{ic2labeldata}.
Since 2016, the major IT companies (\textit{e.g.}, Google~\cite{ic2labeldata}, Microsoft~\cite{miocrosoft_azure_api}, and IBM~\cite{ibm_imgcap_api}) have released and continuously improved their own IC systems.
The leading company of Geographic Information System (GIS), Ersi, has integrated image captioning into its famous GIS framework (\textit{e.g.}, Arcgis\footnote{https://developers.arcgis.com/python/guide/how-image-captioning-works/}) to generate the captions for remote sensing images. 
% \ph{a paragraph about neural networks can produce errors, and some real-world examples of caption errors, and their impact, to motivate our work.}


% \begin{figure}[t]
% 		\centering
% 		\includegraphics[width=1\linewidth]{Figs/real-synthesized.pdf}
% 		\caption{A real image and a synthetic image and their captions.}
% 		\label{fig:real_syn}
% \end{figure}

Despite its wide adoption in various applications, modern IC system could return incorrect captions due to the complexity of deep neural networks and the labeling errors in training datasets, leading to the omission of important objects, deep misunderstanding, and even threats to personal safety~\cite{news_1_ai_nodate,ic2impariment,schroeder_microsoft_2016}. According to the "report on vision"~\cite{organization_world_2019}, more than 2.2 billion people around the world have vision impairment and they are expected to benefit greatly from AI-assistants in which IC is often a major component~\cite{ic2impariment,ic2impariment_2}. However, the embedded IC systems sometimes fail to generate the correct captions~\cite{news_1_ai_nodate}, which make the AI-assistants return misleading message to the visually-impaired users, posing threat to their personal safety. An image of the former U.S. president Barach Obama and his wife was captioned "a man in suit and tie talking on a cell phone"~\cite{schroeder_microsoft_2016}, leading to misunderstanding and potential negative social impact. Thus, assuring the reliability of IC systems is an important endeavor.
% misleading weather reports, distorted news content, and ethical problems~\cite{news_1_ai_nodate, schroeder_microsoft_2016}. For example, one failure case mentioned in a report from Mashable~\cite{schroeder_microsoft_2016} is more ridiculous, that a woman hugging with her husband is captioned as a cell phone, which is disrespectful.

%  For example, a report from CAROL VAN NATTA~\cite{news_1_ai_nodate} shows that an IC system mistakenly captions cats as elephants and fails to depict the seal lions on the beach. 
% Many web APIs: Microsoft’s Azure Cognitive Services\footnote{https://azure.microsoft.com/en-us/services/cognitive-services/}, IBM MAX Image Caption Generator\footnote{https://developer.ibm.com/exchanges/models/all/max-image-caption-generator/}, Neural-Talk-2\footnote{https://deepai.org/machine-learning-model/neuraltalk} \pj{make these links references, and cite the appropriate ones in the previous paragraph}, and image captioning methods~\cite{karpathy2015deep, vinyals_show_2015, xu_show_2015, li_oscar_2020, hu_vivo_2020, zhang_vinvl_2021} have shown great image captioning result in their demos, among which VIVO~\cite{hu_vivo_2020} even claims that it surpasses the human CIDER~\cite{vedantam2015cider} score in a challenge task Nocaps~\cite{agrawal2019nocaps}. 
% Naturally it raises questions, to what extent would the caption models be good enough? Or what capabilities the caption models need to have before they are finally released as commercial software?

% \pj{we should not ask these questions as we cannot answer them directly based on our results.}

% As far as we know, image captioning models give ridiculous in certain corner-case testing data. E.g., when two objects are overlapped with each other, as shown in Fig.~\ref{fig:failurecase1}, a cat overlapped with a zebra may be captioned as a zebra or just be omitted by some image captioning models. This kind of error may cause disastrous results in several settings, and we will explain the damage by several examples and why it is significant to build a testing mechanism for image captioning models. Firstly, a person may get wrong idea of pictures or photos shared by their friends on Facebook or Instagram if the Image Captioning Software they use gives improper depictions.
% IC systems are widely adopted to various utilities. Here are three examples to explain our motivation to design the metamorphic testing method {\methodname} for IC systems. Firstly, people with visual impairment may get wrong information of images or photos if the IC software passes inadequate captions to the Text-to-Speech Reader. According to world vision report~\cite{organization_world_2019}, at least 2.2 billion people around the world have a vision impairment. Promoting the equity of them is one reason of our strong motivation. Secondly, researchers who use IC Software as an assistant to help them analyze the Animal manner may miss some essential information if the software omits some important details or recognize certain animal as another species. Thirdly, explorers who use a GIS system with integrated IC Software~\cite{lu_exploring_2017, qu_deep_2016} as their guidance system could be misguided and endangered in the wrong exploration route if the IC Software improperly depicts remote sensing images of landform.  \pj{merge this paragraph and the previous paragraph. Focusing on explaining the serious impact of IC errors. give at most 2 detailed examples.}

% With the developing of deep learning software and its widespread deployment, the corresponding testing methods also achieve great progress. 

There remains a dearth of automated testing methods for IC systems because the problem is quite challenging.
First, modern IC systems are approaching human-level performance on the existing human-labeled test sets. Thus, test sets of high quality are lacking. 
Second, traditional code-based testing approaches~\cite{romdhana2021cosmo, viticchie2016assessment, ceccato2014family} are not suitable for testing IC systems because the logics of IC systems are mainly encoded in the underlying neural networks with millions of complex parameters, rather the source code. Third, existing testing approaches for computer vision (CV) tasks~\cite{wang2020metamorphic, tian2020testing} typically assume simpler output formats (\textit{e.g.}, class labels), which cannot work well in testing IC systems whose output (\textit{i.e.}, a sentence) is significantly more complex; while existing testing approaches for natural language processing (NLP)~\cite{sun2020automatic,he2020structure,he2021testing} tasks heavily rely on the perturbation of chars or words in the input, which is infeasible for IC systems whose input are images.  
% Thus, it is hard to both synthesize testing data for a comprehensive testing, and get ground truth for these synthesized data.

% There are multiple testing methods well designed for Computer Vision (CV) tasks such as Auto-Driving, Object Detecting, and for Natural Language Processing (NLP) tasks such as machine translation.
% However, there is a dearth of testing methods for multi-modal tasks because it is quite challenging. Image Captioning task is a typical multimodal task that converts image information to text information. The input of IC software is image which is continuous data form and the output is Natural Language which is discrete, increasing the difficulty to test IC systems compared to pure CV and NLP. E.g., CV tasks can easily obtain the Ground Truth of the images after perturbation while it is laborious to get the ground truth of captions of the images after perturbation. The target of IC is to convert the continuous image data into discrete natural language data while retaining the important information of the salient objects along with their manners and relationships, where the objects in IC's input data domain can overlap with each other but the same objects in IC's output domain are discrete words. Generally, NLP testing methods focus on how the change of source text will affect the target text, which are both discrete. However, there doesn't exist a scheme to examine the interaction between semantic information in continuous image data and discrete natural language data.

% \begin{figure*}[ht]
% 		\centering
% 		\includegraphics[width=1.0\linewidth]{Figs/MRs_Show.pdf}
% 		\caption{ Examples of background images, generated images, and the corresponding captions. Words of salient objects are marked in blue. Words indicating the violation of {\methodname}'s MRs are marked in red.}
% 		\label{fig:how_MRs_work}
% \end{figure*}

To tackle these challenges, we introduce {\methodname}, a simple, widely-applicable metamorphic testing methodology for validating IC systems. The input of {\methodname} is a list of unlabeled images, while its output is a list of suspicious issues, where each suspicious issue contains a pair of images and their captions.   
The core idea of {\methodname} is that the object names should exhibit directional changes after object insertion. We realize this idea by two metamorphic relations (MRs): (1) \textit{object appearance}: only the original objects and the inserted objects should appear in the caption of the generated image; (2) \textit{singular-plural form}: both the original objects and the inserted objects should be illustrated by words of a proper singular-plural form. 
Fig.~\ref{fig:how_MRs_work} presents two suspicious issues returned by our approach.
The first issue was reported because the inserted bird was captioned into a "person", violating the first MR; while the second issue was reported because the noun "cow" was not in singular form, violating the second MR. Specifically, {\methodname} automatically extracts objects from images by Yolact++~\cite{bolya2020yolact++}, an advanced real-time image segmentation technique. The extracted object will be inserted into randomly selected images (\textit{i.e.}, background images). This is a challenging step because the inserted object should avoid affecting the saliency of the existing objects, which has been tackled by our novel object resizing and location tuning algorithms.
% \bx{how to emphasize the significance of our insert method} 
The background image and the newly generated image form an image pair. If the captions of this image pair returned by the IC system violate any of the MRs, the image pair and the corresponding captions will be reported as a suspicious issue. 
% Toward this end, a POS tagging technique~\cite{marcus1993building} has been employed to identify the text counterpart of the objects from a caption.
% generates the test data by inserting a single object to the background image while promoting the saliency of the original objects in the background image, and then use our proposed metamorphic relations (MRs) to check if the IC results of the synthesized image and the corresponding background image are constituent-invariant. 
% Considering that target of IC is to caption the salient objects, we have two strategies: (1) make sure the inserted object doesn't overlap with the original objects in the background images, (2) let the inserted objects be overlapped with the original objects while controlling the overlapping ratios between the inserted objects and the original objects. 

% {\methodname} circumvents the direct testing of the output captions produced by IC systems, but testing the MRs of a pair of captions for the background image and synthesized image. We use treebank-specific POS(XPOS)~\cite{marcus1993building} to analyze the caption pair, and report any issues that violate the MRs.
We apply {\methodname} to test one paid IC service, \textit{i.e}., Microsoft Azure Cognitive Services~\cite{miocrosoft_azure_api} and five popular IC models, \textit{i.e.}, Show, Attend and Tell~\cite{xu_show_2015}, $Oscar_B$, $Oscar_L$~\cite{li_oscar_2020}, $VinVL_B$, $VinVL_L$~\cite{zhang_vinvl_2021}. 
% We also apply {\methodname} to test five popular IC models, which are attention-based IC model proposed by Xu et al.~\cite{xu_show_2015}, $Oscar_B$ and $Oscar_L$~\cite{li_oscar_2020}, $VinVL_B$ and $VinVL_L$~\cite{zhang_vinvl_2021}, respectively. 
{\methodname} successfully reports 16,825 erroneous issues in total with high precision of 84.9\%-98.4\%, revealing 17,380 captioning errors. The errors include misclassification, omission, and incorrect quantity. To better understand the reported errors, we visualize the attention masks of the object, which helps us explore the potential root causes behind. Furthermore, we adapt {\methodname} to detect labeling errors in MS COCO Caption, a widely-used standard IC dataset, which reports 151 incorrect labels in the training set, demonstrating {\methodname}'s wide applicability. The source code is also released for reuse~\cite{metaic}. In summary, this paper makes the following main contributions:
\begin{itemize}
    \item It introduces {\methodname}, the \textit{first} metamorphic testing methodology for validating image captioning systems.
    \item  It describes a practical implementation of {\methodname} by adapting Yolact++~\cite{bolya2020yolact++} to extract objects and developing a new object insertion technique that allows flexible insertion position and overlapping area.
    \item It presents the evaluation of {\methodname} that successfully reports 16,825 erroneous issues in one industrial IC service and five SOTA IC models with high precision, and find a total number of 17,380 captioning errors.
    \item It discusses the error categories found by {\methodname}, the exploration of root causes, and the potential of adapting {\methodname} to detect labeling errors in widely-used image captioning datasets.
\end{itemize}
 

% To validate how the semantic information of objects in image data form affect the captions produced by IC software, we let the inserted object 
% Here needs tobackg be examined carefully.
% \begin{figure}[ht]
% 		\centering
% 		\includegraphics[width=0.95\linewidth]{Figs/Figs_failurecase1.pdf}
% 		\caption{A failure case where image captioning web APIs fails}
% 		\label{fig:failurecase1}
% 	\end{figure}

% \ph{a paragraph about why testing image captioning is difficult, challenges}

%Difficult as it is to test how well can a child give a brief depiction of an image, it is also a hard task for researchers to test 

% There remains a dearth of automated testing methods for Image Captioning Software due to its challenge. Firstly, 

% The research of image captioning combines the techniques of Computer Vision(CV) and Natural Language processing(CV), which attracts less interest compared with single task of CV or NLP. Meanwhile, due to its complexity,it is more difficult to design a mechanism which will make the image captioning models fail to give proper depiction of the input images. Unlike image captioning, the attack to the image classification has gained more attention and better progress. There are black-box attack methods 

% No matter in what form, current image captioning models are in one rule, they first extract the 

% When people explain an image or a painting which have several objects overlapped with each other, there is a need for extra logic relationship to proceed the situation where two or more objects are close or overlapped with each other. 

% \ph{a paragraph about the core insights and key implementation details}

% \ph{a paragraph about our experimental results}

==> ISSTA2022_IC (2)/Methodology.tex <==
\section{Approach and Implementation}\label{sec:method}

% \begin{figure*}[t]
% 		\centering
% 		\includegraphics[width=1.0\linewidth]{Figs/framework.pdf}
% 		\caption{Workflow of {\methodname}}
% 		\label{fig:framework}
% 	\end{figure*}

This section introduces {\methodname} and its implementation details. Inspired by the goal of IC that the salient objects in an image should be captioned properly, the core idea of {\methodname} is: the object names should exhibit directional changes after object insertion.
% design {\methodname} to \bxtext{test the IC systems concerning the depiction of the significant objects in the caption}.
The input of {\methodname} is a list of unlabeled images and the output is a list of suspicious issues, where each issue contains the original image, a generated image with an inserted object, and their corresponding captions returned by the IC software under test. Fig.~\ref{fig:framework} illustrates the overview of {\methodname}, which carries out the following four steps:
\begin{enumerate}
    \item \textit{Object extraction}. We extract salient objects from an existing dataset by an instance segmentation algorithm, which collectively form an object pool.
    \item \textit{Object insertion}. For each unlabeled image (\textit{i.e.}, background image), we randomly select an image (\textit{i.e.}, object image) from the object pool and insert it into the background image via novel object resizing and location tuning algorithms.  
    \item \textit{Caption collection}. We collect the captions for the background image and the generated image from the IC system under test.
    \item \textit{Error detection}. We focus on the key constituents in the two captions and report a suspicious issue if the captions violate at least one of our MRs.
\end{enumerate}

\subsection{Object Extraction}
% Firstly we randomly choose an image from the test dataset of MS COCO Caption~\cite{chen2015microsoft} as the background, and then choose an object to be inserted into the background image. In order to get the high-quality object, we collect an object image pool from Flickr~\cite{flickr}, and use an advanced real-time instance-segmentation method Yolact++~\cite{bolya2020yolact++} to extract the standalone object considering both the precision and efficiency. 

% We use Yolact++~\cite{bolya2020yolact++} to extract the standalone object from the image, and categorize them for the usage in the object insertion module.
To realize object insertion, we need to prepare a pool of object images. Thus, the first step of {\methodname} is to extract object images from an image dataset. 
% producing high-quality object instances and put them into separate categories.
Although object extraction has long been a challenging task, deep learning-based object segmentation models~\cite{bolya2019yolact, bolya2020yolact++, he2017mask, li2017fully} provide a feasible solution because these models can extract high-quality objects efficiently. 

In our implementation, we adopt Yolact++~\cite{bolya2020yolact++}, the SOTA real-time object segmentation method because it achieves decent performance in terms of both precision~\cite{he2017mask, li2017fully} and efficiency~\cite{uhrig2018box2pix,bolya2019yolact,bolya2020yolact++}. Yolact++ predicts mask prototypes and per-instance mask coefficients in parallel, and linearly combines them to form the final instance masks. 
Thus, Yolact++ model can achieve 34.1 mAP on MSCOCO~\cite{lin2014microsoft} at 33.5 fps while keeping the close performance of the SOTA approaches. As shown in Fig.~\ref{fig:how_yolact++_works}, Yolact++ generates the masks and identifiers of the airplanes in the images, based on which we can extract the objects accordingly and put them into a certain category (\textit{e.g.}, airplane).

\begin{figure}[ht]
		\centering
		\includegraphics[width=1.0\linewidth]{Figs/Yolact++.pdf}
		\caption{An example of object extraction via Yolact++.}
		\label{fig:how_yolact++_works}
\end{figure}



\subsection{Object Insertion}
Once we have constructed an object pool, we randomly select an object image (\textit{e.g.}, the cow in Fig.~\ref{fig:framework}) from the pool and insert it into a random background image. In this process, we need to address three main issues: (1) how to resize the object image to avoid being too big or too small compared with the salient objects in the background image; (2) how to find a suitable location for insertion; and (3) how to allow reasonable overlap between the object image and the original objects in the background image. In the following, we will introduce our specially-design object resizing and location tuning algorithm and how these algorithms provide us with the flexibility of overlapping area configuration.



% Firstly we choose a maximum overlapping ratio $ratio_{max}$, e.g. $45\%$, then we use set the number $n$ of ratios, e.g. 4, thus the $j^{th}$ ratio $ratio_j$ corresponds to the overlapping ratio of $(ratio_{max}/n)*(j-1)$.
\subsubsection{Object resizing.}
The goal of object resizing is to resize the object image from the original size $(h, w)$ to a new size $(h', w')$, where $h$ and $h'$ refer to their heights and $w$ and $w'$ refer to their widths. {\methodname} is based on the assumption that the inserted object is a salient object and it should not affect the saliency of the objects in the background image. Thus, the resized object image should not be too small nor too big. 
Our object resizing algorithm is illustrated by Fig.~\ref{fig:resizing_show}.
% As illustrated by Fig.~\ref{fig:resizing_show}, our object resizing algorithm can suggest a series of object area sizes within a reasonable range $[S_{min}, S_{max}]$.
To figure out the feasible $(h', w')$, we first determine the area size $s\approx h'\times w'$ by randomly selecting a value from range $[S_{min}, S_{max}]$, where $S_{min}$ and $S_{max}$ are calculated as follows:
\begin{equation}
    \begin{aligned}
    S_{min}& = \alpha*S(b) \\
    S_{max}& = \beta*S(b) \\
    \end{aligned}
\end{equation}
$\alpha$ and $\beta$ are hyper-parameters that we manually set based on empirical experience; $S(b)$ is a normalized value that reflects the area size of the objects in the background image. Specifically, $S(b)$ is calculated by $Softmax$ function as follows:

%下面的ai要思考一下怎么写
\begin{equation}
    \begin{aligned}
    S(b)& = \sum_{i=1}^{N}{ ( Softmax( \frac{a_i}{s_b} )*a_i} ) \\
    Softmax(x_i)& = \frac{e^{x_i}}{\sum_{j=1}^{N}e^{x_j}} \\
    \end{aligned}
\end{equation}
where $a_i$ is the area size of the $i$-th original objects in the background image $b$; $s_b$ is the area size of $b$; $N$ is the number of objects in $b$.  
After randomly selecting an area size $s$ from the interval $[S_{min}, S_{max}]$, we calculate
% we expect that the resized object image is in a similar size as $s$, i.e., $h'\times w'\approx s$. Specifically, 
$(h', w')$ as follows:
\begin{equation}
    \begin{aligned}
    (h', w')& = (h*\sqrt{\frac{s}{h*w}}, w*\sqrt{\frac{s}{h*w}} ) \\
    % s& = Random(S_{min}, S_{max}) \\
    \end{aligned}
\end{equation}

We denote $a_{max}$ as the area size of the largest object in $b$. Empirically when $\frac{a_{max}}{s_b}$ < $40\%$, we set $\alpha$, $\beta$ as 0.8 and 1.3, respectively; otherwise, we set $\alpha$, $\beta$ as 0.1 and 0.37, respectively.

\begin{figure}[ht]
		\centering
		\includegraphics[width=0.9\linewidth]{Figs/resizing_show.pdf}
		\caption{An example of object resizing.}
		\label{fig:resizing_show}
\end{figure}

\subsubsection{Location tuning.}
After resizing the object image, we need to select suitable locations in the background image for object insertion. {\methodname} provides a flexible setting on the overlapping ratio between the inserted object and objects in the background image. Specifically, {\methodname} can generate $n$ images with different overlapping ratios, which are randomly selected from $n$ ratio intervals given a maximum overlapping ratio $ratio_{max}$. The intervals for the overlapping ratios are calculated as follow:
\begin{equation}
    interval_i = 
    \begin{cases}
    [0] & \text { if } i = 0 \\ 
    ( \frac{ratio_{max}}{n-1} * (i-1), \frac{ratio_{max}}{n-1} * (i)  ] & \text { if } i>0
    \end{cases}
\end{equation}

% (intervals: [0] and ($i*\frac{ratio_{max}}{n-1}$, $(i+1)*\frac{ratio_{max}}{n-1}$]) 
For example, if we set $ratio_{max}=0.45$ and $n=4$, we will have four intervals: \textit{i.e.}, [0], (0, 0.15], (0.15, 0.3], (0.3, 0.45]), where "[0]" indicates that the inserted object should not overlap with any of the objects in the background image.
% Since the location directly affects the overlapping area between the inserted object $o$ and the objects in the background image, we first determine the overlapping ratio between the inserted object  and the original objects in the background image. 
% The setting of the overlapping ratio contains two parts: (1) the overlapping ratio between the inserted object and the largest object in the background image, (2) the overlapping ratios between the inserted object and the other objects in the background image except for the largest object. 
% We start by choosing a maximum overlapping ratio $ratio_{max}$ (e.g. 45\%) and the number $n(n\geq 3)$ of ratios (e.g. 4), where the $i$-th overlapping ratio $ratio_i$ can be calculated by $(ratio_{max}/n)*(i-1)$ for $i\geq1$. 
% For example, if we set $ratio_{max}=0.45$ and $(n=3)$, {\methodname} will be configured to have four overlapping area intervals: [0], (0, 0.15], (0.15, 0.3], (0.3, 0.45], where "[0]" indicates that the inserted object should not overlap with any of the objects in the background image. 
The overlapping ratio between two objects is the overlapping ratio between the bounding boxes of the inserted object and that of the objects in the background image. Specifically, the overlapping ratio $O_j$ is defined as:
% Based on our empirical observation of the object insertion process, we recommend $n=3$ to be the number of overlapping ratios that leads to diverse kinds of generated images.
% Specifically, for $i=0$, we set $ratio_0=0$, which means that the inserted object doesn't overlap with the original objects in $b$.
\begin{equation}
    O_j = \frac{A_j\cap A_{obj}}{A_j},
\end{equation}
where $A_j$ is the region of the $j$-th object in the background image, $A_{obj}$ is the region of the inserted object $obj$. 

% Now we have introduced the overlapping ratio intervals and how to calculate the overlapping ratios. 
For each of the ratio intervals, {\methodname} generates one synthetic image by selecting a location $(x, y)$ for object image insertion, leading to overlapping ratio $O_j$ within the interval for all the objects. 
To ensure the overlapping ratio while keeping the saliency of the original objects, {\methodname} requires: (1) $O_j$ should be in the ratio interval if the $j$-th object is the largest object in the background image (Rule $R_1$); (2) otherwise, $O_j$ should be less than or equal to the upper bound of the ratio interval Rule $R_2$.
% When searching for a suitable location for insertion, {\methodname} need to obey several heuristic rules. 
% To better explain the process, we denote $A_{max}$ as the region of the largest original objects, the $O_r$ between the inserted object and that of the largest object in the background image should obey rule $R_1$ that:
% \begin{equation}
%     \begin{aligned}
%     O_r& == ratio_i & i = 0, \\
%     ratio_{i-1}& \leq O_r \leq ratio_i &  1 \leq i\leq n-1.  
%     \end{aligned}
% \end{equation}
% \begin{equation}
%     \begin{aligned}
%     O_r& == ratio_i & i = 0, \\
%     ratio_i& < O_r \leq ratio_i & i=1, \\
%     ratio_i& \leq O_r \leq ratio_i &  2 \leq i\leq n-1.  
%     \end{aligned}
% \end{equation}


% Meanwhile, to promote the saliency of the other original objects $A_k$ except for $A_{max}$, the $O_r$ between the inserted object and that of these objects should obey rule $R_2$ that:
% \begin{equation}
%     \begin{aligned}
%     O_r& == ratio_i & i = 0, \\
%     O_r& \leq ratio_i & i\geq 1.
%     \end{aligned}
% \end{equation}

% During the object insertion, we set $n$ different overlapping ratios for the object insertion, thus achieving a more comprehensive testing of the IC systems.

% \bx{The object location is the last step in the object insertion, and the most complicated one.} 
% Following these rules, we start from finding a coordinate that leads to the maximum overlapping ratio $ratio_{max}$, and then use this coordinate and the coordinate of the centroid of the largest object in the background image to construct a search interval, as shown in Fig.~\ref{fig:insert_example} (a). This search interval facilites the generation of images with other overlapping ratios.

% Given the size of the inserted object $obj$ and $n$ overlapping ratios $\{ratio_0, ...ratio_{n-1}\}$, we need to find the location for insertion and further generate a synthesized image under each ratio value. During the search of a location coordinate $(x_i, y_i)$ to paste the inserted object $obj$, we need to make sure that it satisfies $R_1$ and $R_2$ while keeping the search process efficient, which is very challenging.
It is challenging to select suitable positions that obeys rules $R_1$ and $R_2$ in an efficient manner because there could be multiple objects in a background image, where each poses an overlapping constraint according to the rules.
To tackle this challenge, we develop a two-step algorithm. We first search a suitable coordinate for object insertion that allows an overlapping ratio in $interval_{n-1}$, \textit{e.g.}, (0.3, 0.45] when $ratio_{max}=0.45$ and $n=4$. Then we searches the suitable positions for other ratio intervals only along a line instead of all possible positions. Alg.~\ref{alg:location} presents pseudo-code.
% To illustrate the algorithm, we use position searching with an overlapping interval (0, 0.15] as an example (Fig.~\ref{fig:insert_example}).
% we develop an algorithm to determine the coordinate given a $ratio_i$. This algorithm contains two steps for each ratio value. In the following we introduce the process of finding the location for $ratio_1=0.15$, which is illustrated by Fig.~\ref{fig:insert_example}. Specifically, the background image contains a zebra and a cat while and we intend to find a location for inserting a dog with $ratio_1=15\%$ ($n=4$, $ratio_{max}=45\%$).

% We start from finding the location for $ratio_{n-1}$, i.e., the largest overlapping ratio. 
\textbf{Step 1}: We randomly choose a coordinate $(x_{n-1}, y_{n-1})$ in the background image for object insertion for $interval_{n-1}$ , and check if it obeys $R_1$ and $R_2$ (line 3-7).
If not, {\methodname} calculates a new image size using our image resizing technique, generates a new coordinate $(x, y)$ randomly, and check its compliance with $R_1$ and $R_2$ again. We keep generating new image sizes and coordinates until they obey $R_1$ and $R_2$ or we try $c_1$ times, where $c_1$ is a pre-defined threshold (line 7-11). 
% Fig.~\ref{fig:insert_example}~(a) illustrates the result of this step, where point ``S" is the position found.
% We set a patience value $c_1$ for this algorithm, when \textit{step}-1 is performed for more than $c_1$ times, we randomly select a new inserted object, and then perform \textit{step}-1 again. Finally, we find a point $S$ of coordinate $(x_{n-1}, y_{n-1})$ that meets the satisfaction for $ratio_{n-1}$ (Fig.~\ref{fig:insert_example} (a)).

\textbf{Step 2}: After calculating the coordinate (\textit{e.g.}, point $S$ in Fig.~\ref{fig:insert_example}~(a)) for $interval_{n-1}$, we continue to search for the object insertion coordinates under the remaining ratio intervals. Instead of utilizing the strategy in \textit{step-1} to find a new coordinate, which is time-consuming, we search the coordinate along a line. We denote the centroid coordinate of the largest object in background image as $(x_{max}, y_{max})$, which is point $A$ in Fig.~\ref{fig:insert_example}~(a) (line 17). We construct a line $L$ (red lines in Fig.~\ref{fig:insert_example}) by connecting point $(x_{max}, y_{max})$ and point $(x_{n-1}, y_{n-1})$ and extend the line to point $(x_{bound}, y_{bound})$ (point $B$ in Fig.~\ref{fig:insert_example} (a)), where $(x_{bound}, y_{bound})$ is the farthest coordinate on $L$ keeping the inserted object inside the background image. 
% We adopt binary search in this step, also with a patience value $c_2$. 
% The search interval is on the segment constructed by point $(x_{max}, y_{max})$ and $(x_{bound}, y_{bound})$, where $(x_{bound}, y_{bound})$ is the farthest coordinate on $L$ keeping the inserted object inside the background image, i.e., point $B$ in Fig.~\ref{fig:insert_example} (a). 
{\methodname} then employs binary search to find a suitable coordinate that obeys the rules $R_1$ and $R_2$ along the line (line 18).
% If \textit{step-2} succeeds, coordinates $\{(x_{n-1}, y_{n-1}), ..., (x_0, y_0)\}$ are obtained, which satisfies $R_1$ and $R_2$ for $\{ratio_{n-1}, ..., ratio_0\}$, respectively.
Fig.~\ref{fig:insert_example} (b), (c), (d) demonstrate an example of the binary search process along the line when {\methodname} intends to find a suitable coordinate for ratio interval (0, 0.15]. In the first search, it gets an overlapping ratio that equals to 0\% which is too small. Then it performs the second search and gets the overlapping ratio that equals to 17\%, which violates $R1$. 
Finally, we find coordinate $(x_1, y_1)$ that satisfies $R_1$ and $R_2$ for the ratio interval. We could see that the saliency of the cat is not affected by the inserted dog after insertion. 
For each ratio interval, we allows at most $c_2$ "jumps" in the binary search, where $c_2$ is a pre-defined threshold.
If we cannot find a suitable position for the interval, we will randomly select a new image and starts from \textit{step-1} again.
% The search strategy for other remaining ratios is the same as the one we show in Fig.~\ref{fig:insert_example}, where the only difference is the value of overlapping value we check for $R_1$ and $R_2$.  
% Using our object inserting algorithm, we could synthesize a group of images that look similar but with different overlapping ratios.
% \bx{ Rewriting the inserting method, the start point of another point is not the location of bar3, thus we need to modify it. }

% There is an example shown in Fig.~\ref{fig:insert_example}, in which case we set $n$ as 4 and $ratio_{max}$ as 45\%. we have already got the coordinate $(x_{n-1}, y_{n-1})$ of the inserted object dog with $ratio_{n-1}$, and calculate $(x_{bound}, y_{bound})$ to construct the interval for search. We adopt binary search to search for the corresponding coordinate for $ratio_1=15\%$. \bx{ In the first search, it gets an overlapping ratio that equals to 0\%, then it performs the second search and gets the overlapping ratio that equals to 17\%, which violates the $R1$. Finally, we find an coordinate $(x_1, y_1)$ that satisfies $R_1$ and $R_2$ for $ratio_1$. 

% Besides the largest object, i.e., the zebra, we could see that the saliency of the cat is not affected by the inserted dog during the insertion.} Using our object inserting method, we could synthesize a group of images that look similar but with different $O_r$, as shown in Fig.~\ref{fig:four_similar_img}.

\begin{figure}[t]
		\centering
		\includegraphics[width=1.0\linewidth]{Figs/fig_insert_final.pdf}
		\caption{An example of our location technique.}
		\label{fig:insert_example}
\end{figure}

% \begin{figure*}[ht]
% 		\centering
% 		\includegraphics[width=1.0\linewidth]{Figs/insert_method.pdf}
% 		\caption{An example of our location technique}
% 		\label{fig:insert_example}
% \end{figure*}

% \begin{figure}[ht]
% 		\centering
% 		\includegraphics[width=1.0\linewidth]{Figs/four ratio.pdf}
% 		\caption{A group of synthesized images ($n=4$, $ratio_{max}=45\%$).}
% 		\label{fig:four_similar_img}
% \end{figure}
%for $ratio_i$ when $i\geq1$, we   .the $O_r$ between $obj$ and the largest original object shoud be in the interval $[]$. Meanwhile, the $O_r$ between $obj$ and other original objects should be 

\begin{algorithm}[h]
	\small
	\caption{ An implementation of location tuning }
	\label{alg:location}
	\begin{flushleft}
		\textbf{Input:} the background $b$, a list of object candidates $objects$, number of overlapping ratios $n$, the max overlapping ratio $ratio_{max}$, resizing interval parameters $\alpha$ and $\beta$, patience parameters $c_1$ and $c_2$  \\
		\textbf{Output:} a size for the inserted object, and a list of locations for controlling different overlapping ratios
	\end{flushleft}
	\begin{algorithmic}[1]
		\State $location\_list\leftarrow List(\hspace{0.5ex})$
		\Comment{Initialize with empty list}	
		\For {$obj$ in $objects$}
		\State $coordinate_{max} \gets$  \Call{RandomCoordinate}{ } 
		\State $ObjNewSize \gets$ \Call{RandomSize}{$\alpha$, $\beta$, $obj$, $b$}
		\State $obj \gets$ \Call{Resize}{$obj$, $ObjNewSize$} 
		
		\State $patience_1 \leftarrow$ $0$
		\While {$R_1$ is False or $R_2$ is False for $ratio_{max}$}
		\Comment{Step 1}
		\If{$patience > c_1$ }
		\State break
		\EndIf
		\State $coordinate_{max} \gets$  \Call{RandomCoordinate}{ }
		\State $patience_1+=1$
		\EndWhile

		\For {i in range(0,n-2)} 
		\Comment{Step 2}
		\State $patience_2 \leftarrow$ $0$
		\While {$R_1$ is False or $R_2$ is False for $ratio_{i}$}
		\If{$patience > c_2$ }
		\State break
		\EndIf
		\State $centroid \gets $ \Call{Coordinate}{LargestObjOf(b)}
		\State $coordinate_{i} \gets$ \Call{BinarySearch}{$centroid$, Boundary(b)}
		\State $patience_2+=1$
		\EndWhile
		\State $location\_list$.append($coordinate_{i}$)
		\EndFor
		\If {$Length(location\_list)==n$}
		\State break
		\EndIf
		\EndFor
		\State \Return $ObjNewSize$, $location\_list$
		
	\end{algorithmic}
\end{algorithm}

\subsection{Caption Collection}
After object insertion, {\methodname} constructs image pairs, where each pair contains the background image and a corresponding synthetic image. These images will be input to the IC system under test and the returned captions will be collected. In this paper, we test one paid IC service, \textit{i.e.}, Microsoft Azure Cognitive Services~\cite{miocrosoft_azure_api}, and five popular IC models, \textit{i.e.}, Attention~\cite{xu_show_2015}, $Oscar_B$, $Oscar_L$~\cite{li_oscar_2020}, $VinVL_B$, $VinVL_L$~\cite{zhang_vinvl_2021}. For the paid IC service, we invoke the API provided by Microsoft Azure Cognitive Services~\cite{miocrosoft_azure_api}. For the IC models, we use the open-source code provided by the authors and train our own IC models following the exact description in the original papers.



% algorithm template
% \begin{algorithm}[h]
% 		\small
% 		\caption{RTI implemented as {\implement}.}
% 		\label{alg:rti}
% 		\begin{flushleft}
% 			\textbf{Require:} $source\_sents$: a list of sentences in source language \\
% 			\hspace{9ex} $d$: the distance threshold \\
% 			\textbf{Ensure:} $suspicious\_issues$: a list of suspicious pairs
% 		\end{flushleft}
% 		\begin{algorithmic}[1]
% 			\State $suspicious\_issues\leftarrow List(\hspace{0.5ex})$
% 			\Comment{Initialize with empty list}
% 			\ForAll{\textit{source\_sent} in \textit{source\_sents}}
% 			\State  $constituency\_tree\leftarrow$ \Call{parse}{\textit{source\_sent}}
% 			\State $head \gets constituency\_tree.$head(\hspace{0.5ex})
% 			\State $RTI\_source\_pairs\leftarrow List(\hspace{0.5ex})$ \State \Call{recursiveNPFinder}{$head$, List(\hspace{0.5ex}), $RTI\_source\_pairs$}
% 			\State $RTI\_target\_pairs\leftarrow$ \Call{translate}{$RTI\_source\_pairs$}
% 			\ForAll{ \textit{target\_pair} in \textit{RTI\_target\_pairs}}
% 			\If{\Call{distance}{$target\_pair$} $> d$}
% 			\State Add $source\_pair$, $target\_pair$ to $suspicious\_issues$
% 			\EndIf
% 			\EndFor
% 			\EndFor
			
% 			\State \Return $suspicious\_issues$
			
% 			\Statex %blank line
% 			\Function{recursiveNPFinder}{$node$,\hspace{0.5ex}$rtis$, $all\_pairs$}
% 			\If{$node$ is $leaf$}
% 			\State \Return
% 			\EndIf
% 			\If{$node$.constituent is NP}
% 			\State $phrase\leftarrow node$.string
% 			\ForAll{$container\_phrase$ in $rtis$}
% 			\State Add $container\_phrase$, $phrase$ to  $all\_pairs$
% 			\EndFor
% 			\State Add $phrase$ to  $rtis$
% 			\EndIf
% 			\ForAll{$child$ in $node$.children(\hspace{0.5ex})}
% 			\State \Call{recursiveNPFinder}{$child$, $rtis.\mathrm{copy}(\hspace{0.5ex})$, $all\_pairs$}
% 			\EndFor
% 			\State \Return $all\_pairs$
% 			\EndFunction
			
			
% 			\Statex %blank line
% 			\Function{distance}{$target\_pair$}
% 			\State $rti\_BOW\gets$  \Call{bagOfWords}{$target\_pair$[0]}
% 			\State $container\_BOW\gets$  \Call{bagOfWords}{$target\_pair$[1]}
% 			\State \Return $|rti\_BOW \setminus container\_BOW|$
			
% 			\EndFunction
% 		\end{algorithmic}
% 	\end{algorithm}

\subsection{Error Detection}
After caption collection, {\methodname} inspects the captions of every image pair and reports them as a suspicious issue if they violate our metamorphic relations (MRs). 
% It is quite challenging to automatically disclose the defects of IC software since it is quite laborious to get the ground truth of the captions. To tackle this test oracle problem, 
{\methodname} provides two MRs. 

\textbf{MR1.} We denote the IC system as $I$, the background image as $b$, the generated image as $i'$, the inserted object as $obj$, the caption pair produced by $I$ are $I(b)$ and $I(i')$.  \textit{MR1} is defined as follows:
\begin{equation}
    Set(I(i')) == Set(I(b)) \cup \{obj\},
\end{equation}
where $Set(I(i'))$ denotes the set of object classes in $I(i')$, $Set(I(b))$ indicates the set of object classes in $I(b)$. 
% If the caption do not violate the first MR, we will check the second MR for the singular-plural form of the objects, which is defined as follows. 

\textbf{MR2.} We use a function $F_*(y)$ to denote the singular-plural form of an object class $y$ in caption $I(*)$, indicating whether the object class $y$'s form is singular or plural. For example, $F_b(dog)$ is the singular-plural form of ``dog" class in the caption of background image $b$.
% and a function $F_{i'}$ to denote the singular-plural form of in $I(i')$. 
% Intuitively, $F_{*}(y)$ indicates whether the object class $y$'s form is singular or plural. 
$C$ denotes the object classes in both $I(b)$ and $I(i')$; $c_k$ is the $k$-th object class in $C$. If the inserted object $obj$ is not in $Set(I(b))$
% , then $Set(I(b))==Set(I(i'))$
, \textit{MR2} requires:
\begin{equation}
    \begin{aligned}
    F_b(c_k) = F_{i'}(c_k), \\
    F_{i'}(obj) = singular.
    % F_i(C_t)& == plural& o \in Set(I(b))&, t=k, \\
    % F_i(C_t)& == singular& o \notin Set(I(b))&, t=k, \\
    % F_i(C_t)& == F_i'(C_t)& t\ne k,
    \end{aligned}
\end{equation}
% where the $k$-th object class in $I(i')$ denotes the inserted object $obj$. $F_i(C_t)$ and $F_i'(C_t)$ denote the singular-plural-form of the $t$-th object class in background image $b$ and synthesized image $i'$.
If the inserted object $obj$ is in $Set(I(b))$, we consider $C'=C\setminus\{obj\}$, where $c_j$ is the $j$-th object class in $C'$. Then the second MR requires:
\begin{equation}
    \begin{aligned}
    F_b(c_j) = F_{i'}(c_j), \\
    F_{i'}(obj) = plural.
    \end{aligned}
\end{equation}
% Intuitively, if the inserted object class already exists in the background image, the object class should be in plural form. Otherwise, the objects in the background image remains its original singular-plural form, while the inserted object class should be in singular form.
If any of the two MRs are violated, the original image, the generated image, and the corresponding captions will be reported as a suspicious issue.
% For simplicity, we use $singular$ and $plural$ to denote the number of the existed objects.

%The two MRs are:(1)the set of object classes in $I(i')$ is the same as the union set of object classes in $I(i)$ and $\{o\}$, (2)after insertion of $o$, the object-noun's form in $I(i')$ should satisfy the condition that:

% \subsection{Analyzing Method}

% However, given an object in the image, it is difficult to locate the corresponding word in the caption. To address this problem,
In our implementation, we mark up the word in caption according to a particular part of speech (POS) via a POS tagging tool, \textit{i.e.}, XPOS~\cite{marcus1993building}. 
% XPOS is trained on a large annotated corpus containing over 4.5 million words in English.
% XPOS contains 36 POS tags and 12 other tags (for punctuation and currency symbols). 
We extract words from the captions whose POS are NN or NNS, corresponding to singular noun or plural noun, respectively. Then we can obtain the a set containing all the object classes in a caption, and construct the mapping for function $F$ which assigns the singular-plural form to the object class in the set. 
% For a pair of images $(i, i')$, we generate a pair of captions $(I(i), I(i'))$ by an IC. We start by checking the first MR, if the caption pair $(I(i), I(i'))$ doesn't violate the first MR, then we will check whether it satisfies the second MR. If $(I(i), I(i'))$ violates any one of the two MRs, we will report it as suspicious issue that has improper caption.
% \subsection{Image/pair generation}
% \subsection{Caption}

% \begin{figure}[ht]
% 		\centering
% 		\includegraphics[width=1.0\linewidth]{Figs/xpos_table.png}
% 		\caption{Table of the Penn Treebank tag set}
% 		\label{fig:xpos_table}
% \end{figure}

% write directly----remains
%************Metamorphic relations(MRs) are necessary properties of the intended functionality of the software to be tested, involving multiple executions of the software. Under the circumstance of metamorphic testing(MT)~\cite{chen2018metamorphic, chen2020metamorphic, segura2016survey}


% \subsection{Object Inserting Method}
% The object inserting method consists of two submodules, which are object extraction and object insertion. \bx{In the object extraction module,  In the object insertion module, we paste the extracted object on the chosen background image to produce the synthesized data. } By using our object inserting method, we could provide ample high-quality testing data for {\methodname}. 

% \subsubsection{Dataset collection}
% We choose background images from the test dataset of Microsoft COCO DATASET~\cite{chen2015microsoft}, and collect typical object images from Flickr and categorize them. For simplicity, we choose 60 classes of objects which only have one word in Microsoft COCO DATASET as our testing domain. 

% Our testing method is to insert object to the background image while promising the saliency of the object. This perturbation method will have the non-local effect which will make the image captioning model give several kinds of errors. 


% We insert our extracted object into the background image and let it be overlapped with the original objects in different overlapping ratios, providing several choices for IC testing task. 
% Meanwhile, we resize the inserted object referring to the size of the original objects to make sure that the inserted one is salient and it doesn't affect the saliency of the original objects in the background image.

==> ISSTA2022_IC (2)/Motivation.tex <==
\begin{figure}[t]
		\centering
		\includegraphics[width=0.95\linewidth]{Figs/real-synthesized.pdf}
		\caption{ A real image, a synthetic image, and their captions. }
		\label{fig:real_syn}
\end{figure}

\section{Preliminaries}\label{sec:pre}
In this section, we first explain the basic concepts that have been used multiple times in the paper. Then we introduce two mainstream image captioning models: CNN-RNN-Based IC and Vision-Language Pre-Training IC.

% Modern IC systems have tackled these problems, with higher precision and lower dependency on handcraft. Two mainstream IC techniques are briefly introduced below.
 


 
\subsection{Basic Concepts}

% To better convey the core idea of {\methodname}, we explain concepts that are used multiple times in the paper. 
Image captioning outputs a depiction of the \textit{salient objects} in a given image (real or synthetic), where salient objects refer to the most noticeable object(s) in the image; and \textit{saliency} reflects whether an object is salient or not. 
For example, in Fig.~\ref{fig:real_syn}, the two people are salient objects in the real-scene image, and the man and the cow are salient objects in the synthetic image. Each object has an \textit{object class}, such as "elephant" and "dog" in Fig.~\ref{fig:how_MRs_work}. In a caption returned by IC software, a salient object is typically illustrated by a noun, whose \textit{singular-plural form} indicates whether the word is a singular noun or a plural noun.

\begin{figure*}[ht]
		\centering
		\includegraphics[width=1.0\linewidth]{Figs/framework.pdf}
		\caption{Overview of {\methodname}.}
		\label{fig:framework}
\end{figure*}


In this paper, we test one IC service and five IC models: Microsoft Azure API~\cite{miocrosoft_azure_api}, Attention~\cite{xu_show_2015}, $Oscar_B$, $Oscar_L$~\cite{devlin2018bert}, $VinVL_B$, $VinVL_L$~\cite{zhang_vinvl_2021}. Specifically, 
Microsoft Azure is short for Microsoft Azure Cognitive services~\cite{miocrosoft_azure_api} and Attention is short for Show, Attend and Tell~\cite{xu_show_2015}. $Oscar_B$ and $VinVL_B$ refer to the IC models adopting the base version of BERT~\cite{devlin2018bert}, while $Oscar_L$ and $VinVL_L$ adopt the large version.





\subsection{Modern Image Captioning Systems}

% Before the wide of adoption of deep neural networks, IC is eachdetections to infer a triplet of scene elements~\cite{farhadi2010every, li2011composing} or a complex graph~\cite{kulkarni2013babytalk} which are then converted to text with the help of templates. Although some IC methods have adopted more powerful language models to text generation~\cite{aker2010generating, elliott2013image, kuznetsova2012collective, kuznetsova2014treetalk, mitchell2012midge}, these approaches are still heavily hand-designed and rigid.

Recently, there are two main lines of IC research: CNN-RNN-Based IC~\cite{xu_show_2015, vinyals_show_2015} and Vision-Language Pre-Training (VLP) IC~\cite{zhou2020unified, hu_vivo_2020, li_oscar_2020, zhang_vinvl_2021}. They both adopt a two-stage framework, using CNNs for feature extraction in the first stage and sequence models caption generation in the second stage. Differently, VLP IC adopts pre-trained models in the second stage, which makes them more efficient and accurate than CNN-RNN-Based IC. In particular, the SOTA VLP IC model VIVO~\cite{hu_vivo_2020} claims that it surpasses human in CIDER score~\cite{vedantam2015cider}. In the following, we elaborate more on these two lines of research.
% transformer~\cite{vaswani2017attention} as their sequence model, which is more efficient than recurrent neural network (RNN), generally they have better performance than CNN-RNN-Based ICs. VIVO~\cite{hu_vivo_2020}, One of the VLP ICs, even mentions that it surpasses the human in CIDER score~\cite{vedantam2015cider}.

 

\subsubsection{CNN-RNN-Based ICs}

% The CNN-RNN-Based ICs form a two-stage pipeline, which 
CNN-RNN-Based IC uses a CNN as the feature extractor and an RNN to generate the captions.  
Specifically, CNN can produce rich representation of an image by embedding it into a fixed-length vector and the representation has been used in various CV tasks~\cite{sermanet2013overfeat}.
% Over the last few years of Deep Learning's high-speed development, it has been convincingly verified that CNN can produce rich representation of the image data by embedding it into a vector with fixed-length, so that the representation can be adopted for various CV tasks~\cite{sermanet2013overfeat}.
Inspired by the great successes of sequence generation in machine translation~\cite{bahdanau2014neural, cho2014learning, sutskever2014sequence}, RNN models~\cite{karpathy2015deep,xu_show_2015,vinyals_show_2015} have been adopted in caption generation in CNN-RNN-Based IC. Attention~\cite{xu_show_2015} first introduces an attention mechanism to image captioning and visualize how the model attends on the salient objects in an image during captioning. 
% Unlike other CNN-RNN-Based ICs that use fully connected layers, this work extract features from a lower convolutional layer, which obtains a correspondence between the feature vectors and specific portions of the 2D images. 
By using a lower convolutional layer rather than fully connected layers in the encoder, the RNN decoder of this method can focus on the most important parts of the image by calculating weights from the feature vectors.
% weighting a subset of all the feature vectors.
As for the second stage, it adopts LSTM~\cite{hochreiter1997long} for caption generation.
% in the second stage and provides two alternative mechanisms for the attention model. 
% The architecture of Show, Attend and Tell is shown in Fig.~\ref{fig:showattend_framework}.

% \begin{figure}[ht]
% 		\centering
% 		\includegraphics[width=1.0\linewidth]{Figs/showattend_framework.png}
% 		\caption{Architecture of Show,attend and tell~\cite{xu_show_2015}}
% 		\label{fig:showattend_framework}
% \end{figure}


\subsubsection{Vision-Language Pre-Training ICs}

VLP ICs also adopts a two-stage pipeline. Differently, they employ more advanced CNNs in the first stage and BERT~\cite{devlin2018bert} in the second stage. With a multi-layer bidirectional Transformer~\cite{vaswani2017attention} as its architecture, BERT uses masked language models to enable pre-trained deep bidirectional representations, which effectively alleviate the extensive manual effort on building task-specific architectures. 

Oscar~\cite{li_oscar_2020} first adopts object tags detected in images as anchor points, which strengthens the learning of semantic alignments between images and texts and significantly enhance its ability to learn the cross-modal representations. 
% By sufficiently utilizing the object tags, Oscar achieves a competent performance in IC task.
Recently, Zhang \textit{et al.}~\cite{zhang_vinvl_2021} propose VinVL, which uses a CNN specially tailored for vision-language tasks. This CNN is pre-trained on a much larger text-image corpora, thus it can capture much more abundant visual features accurately, outperforming other models.




% , and the good performance of BERT used as sequential model in the second stage, The VLP ICs are developing at a high speed and achieve outstanding performance.
% Benefited from the rapidly evolving object-attribute detection models which could provide better image feature extractors in the first stage


% Inspired by the observation that the salient objects in an image can be accurately detected, Li et al.~\cite{li_oscar_2020} propose OSCAR, which uses object tags detected in images as anchor points to strengthen the learning of semantic alignments between images and texts, improving the VLP model's ability to learn the cross-modal representations significantly. To enhance the feature extractor in the first stage, Zhang et al.~\cite{zhang_vinvl_2021} propose VinVL, which uses a large-scale object-attribute detection model based on the ResNeXt-152 C4 architecture that is better designed for Vision-Language tasks and trained on much larger amount of data.

% Oscar_B$ is the IC model with Bert~\cite{devlin2018bert} in Oscar~\cite{li_oscar_2020} base as the language model, $Oscar_L$ is the corresponding IC model using Bert large. $VinVL_B$ is the IC model using Bert base as the language model in VinVL~\cite{zhang_vinvl_2021}, and $VinVL_L$ is the IC model using Bert large as the corresponding language model using Bert large.


% The second concept is the singular-plural form, which we use to denote the number of the object class in the caption. For example, if there is only one horse in the image, the singular-plural form of the object class, i.e., the horse, is singular. Conversely, if there are two or more horses in the image, the singular-plural form of the horse is plural. The concept of singular-plural form is used to implement the second MR we propose. 
% The third concept is the saliency of the object in the images.
% IC software concern much about the saliency of the object in the image, which means the property of whether the object is salient or significant. One core idea of the IC task is that the salient objects of the image need to be depicted in the captions, which is also the basis of the IC task and IC systems.

% Karpathy et al.~\cite{karpathy2015deep} feature a novel ranking model to align parts of visual and language modalities through a multimodal embedding technique, they use a specific region convolutional neural network (RCNN)~\cite{girshick2014rich} as the CNN feature extractor in the first stage, and then use a  bidirectional multimodal RNN architecture to generate the descriptions of visual data.

% Vinyals et al.~\cite{vinyals_show_2015} adopt the CNN architecture which yields the best on the ILSVRC 2014
% classification competition with batch normalization~\cite{ioffe2015batch} in the first stage. Compared to the RNN technique used by Karpathy et al.~\cite{karpathy2015deep}, Vinyals~\cite{vinyals_show_2015}
% adopt a particular form of RNN named Long-Short Term Memory (LSTM), which does well in dealing with vanishing and exploding gradients~\cite{hochreiter1997long}.


% Motivated by BERT's great success in NLP tasks, Zhou et al.~\cite{zhou2020unified} present a Unified Vision-Language Pre-Training (UVLP) model, which unifies the Transformer encoder and decoder into one single model. The input of the model consists of image-region feature which is extracted by a variant of Faster R-CNN~\cite{ren2015faster}, and the associated/target captions. The Faster R-CNN of UVLP uses ResNeXt-101 FPN~\cite{xie2017aggregated} as the backbone, taking the output of the fc6 layer as feature representation for each region and finetuning the fc7 layer. For IC task, it first finetunes the pre-trained UVLP model on the target dataset using the seq2seq objective, then uses greedy search on the validation set and beam research with beam size 5 on the test set. 
% The architecture of UVLP is shown in Fig.~\ref{fig:uvlp_framework}.

% \begin{figure}[ht]
% 		\centering
% 		\includegraphics[width=1.0\linewidth]{Figs/UVLP_framework.png}
% 		\caption{Architecture of UVLP~\cite{zhou2020unified}}
% 		\label{fig:uvlp_framework}
% \end{figure}

==> ISSTA2022_IC (2)/Relatedwork.tex <==
\section{Related Work}\label{sec:related}

%\subsection{Image Captioning}






\subsection{Robust AI Software}
In recent years, deep neural networks have achieved great success in a variety of fields and thus artificial intelligence (AI) software has been widely used in our daily lives. However, AI software can generate erroneous outputs that cause severe accidents and even endanger the users~\cite{accident1,accident2,accident3}. To explore the vulnerability of AI software, a line of research has focused on attacking various AI systems, such as classification systems~\cite{goodfellow2014explaining, luo2018towards, zhao2020towards}, and automatic speech recognition systems~\cite{qin2019imperceptible, carlini2018audio}. These papers fool the AI software with imperceptible perturbations. Meanwhile, to enhance the reliability of AI software, a variety of related topics have been studied, including testing~\cite{du2019deepstellar, gambi2019automatically, henriksson2019towards, he2020structure,he2021testing,Kang2020aa}, online adversarial detection~\cite{ma2019nic, tao2018attacks, wang2019adversarial, gu2019detecting}, and robust training mechanisms for deep neural networks~\cite{kannan2018adversarial, lin2019defensive, madry2017towards, papernot2016distillation}. Most of these methods are white-box, largely dependent on the knowledge of the model internals; while our approach is black-box, which can be easily adapted to test any IC systems.
% needs no model internal details and 

%attack, testing repair *refred icse20-trans
%Machine translation~\cite{He20ICSE}

\subsection{Multimodal Task and Image   Captioning}

% Multimodal machine learning aims to build models that can process and relate, Baltru{\v{s}}aitis et al.~\cite{baltruvsaitis2018multimodal} 
Modality refers to the way in which something happens or being sensed by human. Accordingly, a multimodal task indicates that the task involves more than one modality (\textit{e.g.}, image and text for image captioning). The corresponding AI models need to learn these multimodal signals collectively, which brings new challenges as introduced by Baltru{\v{s}}aitis et al.~\cite{baltruvsaitis2018multimodal}: representation, translation, alignment, fusion, and co-learning. Typical multimodal tasks include speech recognition and synthesis~\cite{hannun2014deep, kalchbrenner2018efficient}, cross-modal retreival~\cite{gao2020fashionbert, vo2019composing}, and image captioning~\cite{xu_show_2015, li_oscar_2020, zhang_vinvl_2021, vinyals_show_2015}. Compared with single-modal systems (\textit{e.g.}, image classifier or machine translation), multimodal systems are more difficult to test because we need to consider the translation from one modality to another and most of the existing testing techniques for single-modal models cannot be used here without non-trivial adaptations.

Recent years have witnessed the blossom of IC systems, where researchers focus on improving the accuracy of IC. For CNN-RNN-Based IC, researchers designed various CNNs and RNNs to enhance the intermediate representation~\cite{karpathy2015deep,vinyals_show_2015,xu_show_2015}. For VLP IC, researchers proposed multiple pre-trained techniques~\cite{zhou2020unified, li_oscar_2020, hu_vivo_2020, zhang_vinvl_2021}. Different from these papers that make effort to achieve high accuracy, {\methodname} aims to improve the robustness of IC. To this end, several papers focus on attacking existing IC models in a white-box manner~\cite{xu2019exact, chen2018attacking, xu2018fooling}, which requires the complete knowledge of underlying networks. Differently, {\methodname} is black-box, which does not rely on model internals, such as network structure and parameters.

% information from multiple modalities

% \subsection{Label errors in dataset}
\subsection{Metamorphic Testing}
Metamorphic Testing (MT) is a general methodology that applies a transformation to test input(s) and observes how the program output turns into a different one as a result~\cite{chen2020metamorphic, segura2016survey, chen2018metamorphic}. The core idea of MT is to verify the MRs between the outputs from multiple runs of the program with different inputs, which is useful when test oracle is lacking. MT is widely adopted in traditional software, such as compilers~\cite{le2014compiler,lidbury2015many}, datalog engines~\cite{mansur2021metamorphic}, and service-oriented applications~\cite{chan2005towards, chan2007metamorphic}. Recently, it has also been used in testing AI software, such as autonomous cars~\cite{tian_deeptest_2018, zhang2018deeproad}, statistical classifiers~\cite{xie2009application, xie2011testing}, object detection~\cite{wang2020metamorphic}, and machine translation~\cite{he2020structure, he2021testing}. In this paper, we propose {\methodname}, a novel, widely-applicable metamorphic testing approach for image captioning.


